Gradient Surgery for Multi-Task Learning

While deep learning and deep reinforcement learning (RL) systems have demonstrated impressive results in domains such as image classification, game playing, and robotic control, data efficiency remains a major challenge. Multi-task learning has emerged as a promising approach for sharing structure across multiple tasks to enable more efficient learning. However, the multi-task setting presents a number of optimization challenges, making it difficult to realize large efficiency gains compared to learning tasks independently. The reasons why multi-task learning is so challenging compared to single-task learning are not fully understood. In this work, we identify a set of three conditions of the multi-task optimization landscape that cause detrimental gradient interference, and develop a simple yet general approach for avoiding such interference between task gradients. We propose a form of gradient surgery that projects a task's gradient onto the normal plane of the gradient of any other task that has a conflicting gradient. On a series of challenging multi-task supervised and multi-task RL problems, this approach leads to substantial gains in efficiency and performance. Further, it is model-agnostic and can be combined with previously-proposed multi-task architectures for enhanced performance.

==> Gradient Surgery for Multi-Task Learning NeurIPS/defs.tex <==
%% editing comment
\newcommand{\cmt}[1]{{\footnotesize\textcolor{red}{#1}}}
\newcommand{\note}[1]{\cmt{Note: #1}}
%\newcommand{\todo}[1]{\cmt{To-Do: #1}}


%% abbreviations
\newcommand{\x}{\mathbf{x}}
\newcommand{\z}{\mathbf{z}}
\newcommand{\y}{\mathbf{y}}
\newcommand{\w}{\mathbf{w}}
\newcommand{\data}{\mathcal{D}}

\newcommand{\etal}{{et~al.}\ }
\newcommand{\eg}{e.g.\ }
\newcommand{\ie}{i.e.\ }
\newcommand{\nth}{\text{th}}
\newcommand{\pr}{^\prime}
\newcommand{\tr}{^\mathrm{T}}
\newcommand{\inv}{^{-1}}
\newcommand{\pinv}{^{\dagger}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\gauss}{\mathcal{N}}
\newcommand{\norm}[1]{\left|#1\right|}
\newcommand{\trace}{\text{tr}}

%% specifics for the paper
\newcommand{\reward}{r}
\newcommand{\policy}{\pi}
\newcommand{\mdp}{\mathcal{M}}
\newcommand{\states}{\mathcal{S}}
\newcommand{\actions}{\mathcal{A}}
\newcommand{\observations}{\mathcal{O}}
\newcommand{\transitions}{\mathcal{T}}
\newcommand{\initial}{\mathcal{I}}
\newcommand{\horizon}{H}
\newcommand{\rewardevent}{R}
\newcommand{\probr}{p_\rewardevent}
\newcommand{\metareward}{\bar{\reward}}

\newcommand{\pihi}{\pi^{\text{hi}}}
\newcommand{\pilo}{\pi^{\text{lo}}}
\newcommand{\ah}{\mathbf{w}}

\newcommand{\loss}{\mathcal{L}}
\newcommand{\eye}{\mathbf{I}}

\newcommand{\model}{\hat{p}}

\newcommand{\pimix}{\pi_{\text{mix}}}

\newcommand{\pib}{\bar{\pi}}
\newcommand{\epspi}{\epsilon_{\pi}}
\newcommand{\epsmodel}{\epsilon_{m}}

\newcommand{\upd}{\mathcal{U}}

\newcommand{\ind}{\delta}

%% math
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\en}{\mathcal{E}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bz}{\mathbf{z}}
\newcommand{\bo}{\mathbf{o}}
\newcommand{\bs}{\mathbf{s}}
\newcommand{\ba}{\mathbf{a}}
\newcommand{\ot}{\bo_t}
\newcommand{\st}{\bs_t}
\newcommand{\at}{\ba_t}
\newcommand{\op}{\mathcal{O}}
\newcommand{\opt}{\op_t}
\newcommand{\kl}{D_\text{KL}}
\newcommand{\tv}{D_\text{TV}}
\newcommand{\ent}{\mathcal{H}}

\newcommand{\bzhi}{\bz^\text{hi}}

==> Gradient Surgery for Multi-Task Learning NeurIPS/experiments.tex <==

\section{Experiments}
\label{sec:experiments}

The goal of our experiments is to study the following questions: (1) Does PCGrad make the optimization problems easier for various multi-task learning problems including supervised, reinforcement, and goal-conditioned reinforcement learning settings across different task families? (2) Can PCGrad be combined with other multi-task learning approaches to further improve performance? (3) \KH{Is the tragic triad of multi-task learning} a major factor in making optimization for multi-task learning challenging? To broadly evaluate PCGrad, we consider multi-task supervised learning, multi-task RL, and goal-conditioned RL problems. \neurips{We include the results on goal-conditioned RL in Appendix~\ref{app:goal-conditioned}.}
%
%
%
%


\neurips{
During our evaluation, we tune the parameters of the baselines independently, ensuring that all methods were fairly provided with equal model and training capacity. PCGrad inherits the hyperparameters of the respective baseline method in all experiments, and has no additional hyperparameters. For more details on the experimental set-up and model architectures, see Appendix~\ref{app:exp_details}.}
The code is available online\footnote{Code is released at \url{https://github.com/tianheyu927/PCGrad}}.



\subsection{Multi-Task Supervised Learning}

%
%
\neurips{To answer question (1) in the supervised learning setting and question (2), we perform experiments on five standard multi-task supervised learning datasets: MultiMNIST, CityScapes, CelebA, multi-task CIFAR-100 and NYUv2. We include the results on MultiMNIST and CityScapes in Appendix~\ref{app:additional_mt_sup_results}.}

\begin{table*}[t]
  \centering
  \scriptsize
  \def\arraystretch{0.9}
  \setlength{\tabcolsep}{0.42em}
    \begin{tabularx}{0.95\linewidth}{ccll*{9}{c}}
  \toprule
 \multicolumn{1}{c}{\multirow{3.5}[4]{*}{\#P.}} & \multicolumn{1}{c}{\multirow{3.5}[4]{*}{Architecture}} & \multicolumn{1}{c}{\multirow{3.5}[4]{*}{Weighting}} & \multicolumn{2}{c}{Segmentation} & \multicolumn{2}{c}{Depth}  & \multicolumn{5}{c}{Surface Normal}\\
  \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-12}
   &\multicolumn{1}{c}{}  &\multicolumn{1}{c}{} & \multicolumn{2}{c}{\multirow{1.5}[2]{*}{(Higher Better)}} & \multicolumn{2}{c}{\multirow{1.5}[2]{*}{(Lower Better)}}   & \multicolumn{2}{c}{Angle Distance}  & \multicolumn{3}{c}{Within $t^\circ$} \\
    &\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{}  & \multicolumn{1}{c}{} & \multicolumn{2}{c}{(Lower Better)} & \multicolumn{3}{c}{(Higher Better)} \\
     & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{mIoU}  & \multicolumn{1}{c}{Pix Acc}  & \multicolumn{1}{c}{Abs Err} & \multicolumn{1}{c}{Rel Err} & \multicolumn{1}{c}{Mean}  & \multicolumn{1}{c}{Median}  & \multicolumn{1}{c}{11.25} & \multicolumn{1}{c}{22.5} & \multicolumn{1}{c}{30} \\
\midrule
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
  &    &Equal Weights   & 14.71  & 50.23   &  0.6481   &  0.2871 & 33.56 & 28.58 & 20.08 & 40.54 & 51.97\\
  $\approx$3 & Cross-Stitch$^\ddagger$    &Uncert. Weights$^*$  &  15.69 &  52.60  &  0.6277   & 0.2702 & 32.69 &  27.26 & 21.63 &  42.84 &  54.45 \\
  &     &DWA$^\dagger$, $T = 2$   & {\bf 16.11} &  {\bf  53.19} & {\bf 0.5922}   & {\bf 0.2611} & {\bf 32.34} & {\bf 26.91} & {\bf 21.81} & {\bf 43.14} & {\bf 54.92} \\
  \cmidrule(lr){2-13}
  &    & Equal Weights &   {\bf 17.72} &  55.32    & {\bf 0.5906}  &  0.2577 & 31.44  & {\bf 25.37}&  \mybox{\bf 23.17} & 45.65 &57.48\\
1.77 & MTAN$^\dagger$ & Uncert. Weights$^*$  &  17.67    &  {\bf 55.61}  &  0.5927    & 0.2592 & {\bf 31.25} & 25.57 & 22.99 & {\bf 45.83} & {\bf 57.67} \\    & &DWA$^\dagger$, $T = 2$   &  17.15    &  54.97 &  0.5956  & {\bf 0.2569} & 31.60 & 25.46 & 22.48 & 44.86 & 57.24 \\
      \cmidrule(lr){2-13}
1.77 & MTAN$^\dagger$+ PCGrad (ours) & Uncert. Weights$^*$  &  \mybox{\bf 20.17}    &  \mybox{\bf 56.65}  &  \mybox{\bf 0.5904}    & \mybox{\bf 0.2467} & \mybox{\bf 30.01} & \mybox{\bf 24.83} & 22.28 & \mybox{\bf 46.12} & \mybox{\bf 58.77} \\
    \bottomrule
    \end{tabularx}
    \vspace{-0.2cm}
         \caption{\footnotesize Three-task learning on the NYUv2 dataset: 13-class semantic segmentation, depth estimation, and surface normal prediction results. \#P shows the total number of network parameters. We highlight the best performing combination of multi-task architecture and weighting in bold. The top validation scores for each task are annotated with boxes. The symbols indicate prior methods: $^*$: \citep{kendall2017multi}, $^\dagger$: \citep{liu2018attention}, $^\ddagger$: \citep{misra2016crossstitch}. Performance of other methods as reported in \citet{liu2018attention}.
     \label{tab:mtl_results_compare}
     }
\end{table*}

\begin{wraptable}{R}{0.5\textwidth}
\vspace{-0.5cm}
%
    \begin{center}
    \begin{small}
    \begin{tabular}{l|c}
    \toprule
        & \% accuracy  \\
      \midrule
      task specific, 1-fc~\citep{rosenbaum2017routing} & 42\\
      %
      task specific, all-fc~\citep{rosenbaum2017routing} & 49\\
      cross stitch, all-fc~\citep{misra2016crossstitch} & 53\\
      %
      routing, all-fc + WPL~\citep{rosenbaum2019routing} & 74.7\\
      %
      independent & 67.7\\
      \midrule
      PCGrad (ours) & 71\\
      routing-all-fc + WPL + PCGrad (ours) & \bf 77.5 \\
      \bottomrule
    \end{tabular}
    \end{small}
    \end{center}
    \vspace{-0.4cm}
    \caption{\footnotesize CIFAR-100 multi-task results. When combined with routing networks, PCGrad leads to a large improvement.}
    \label{tbl:cifar}
%
\end{wraptable}

For CIFAR-100, we follow~\citet{rosenbaum2017routing} to treat 20 coarse labels in the dataset as distinct tasks, creating a dataset with 20 tasks, with 2500 training instances and 500 test instances per task. We combine PCGrad with a powerful multi-task learning architecture, routing networks~\citep{rosenbaum2017routing, rosenbaum2019routing}, by applying PCGrad only to the shared parameters. \icmllast{For the details of this comparison, see Appendix~\ref{app:sl_details}.} As shown in Table~\ref{tbl:cifar}, \arxiv{applying PCGrad to a single network achieves 71\% classification accuracy, which outperforms most of the prior methods such as cross-stitch~\citep{misra2016crossstitch} and independent training, suggesting that sharing representations across tasks is conducive for good performance. While routing networks achieve better performance than PCGrad on its own, they are complementary: combining PCGrad with routing networks leads to a $2.8\%$ absolute improvement in  test accuracy.} %

We also aim to use PCGrad to tackle a multi-label classfication problem, which is a commonly used benchmark for multi-task learning. In multi-label classification, given a set of attributes, the model needs to decide whether each attribute describes the input. Hence, it is essentially a binary classification problem for each attribute. We choose the CelebA dataset~\cite{liu2015deep}, which consists of 200K face images with 40 attributes. Since for each attribution, it is a binary classfication problem and thus we convert it to a 40-way multi-task learning problem following \citep{sener2018multi}. We use the same architecture as in \cite{sener2018multi}.

We use the binary classification error averaged across all $40$ tasks to evaluate the performance as in~\cite{sener2018multi}. Similar to the MultiMNIST results, we compare PCGrad to \citet{sener2018multi} by rerunning the open-sourced code provided in~\cite{sener2018multi}. As shown in Table~\ref{tbl:celeba}, PCGrad outperforms~\citet{sener2018multi}, suggesting that PCGrad is effective in multi-label classification and can also improve multi-task supervised learning performance when the number of tasks is high.

\begin{table}[h]
    \begin{center}
    %
    %
    \begin{small}
    \begin{tabular}{l|c}
    \toprule
        & average classification error  \\
      \midrule
      \citet{sener2018multi} & 8.95\\
      \midrule
      PCGrad (ours) & \bf 8.69 \\
      \bottomrule
    \end{tabular}
    \end{small}
    \end{center}
    \caption{\footnotesize CelebA results. We show the average classification error across all 40 tasks in CelebA. PCGrad outperforms the prior method~\citet{sener2018multi} in this dataset.}
    \vspace{-0.4cm}
    \label{tbl:celeba}
\end{table}


Finally, we combine PCGrad with another state-of-art multi-task learning algorithm, MTAN~\citep{liu2018attention}, and evaluate the performance on a more challenging indoor scene dataset, NYUv2, which contains 3 tasks: \icml{13-class semantic segmentation, depth estimation, and surface normal prediction}. We compare MTAN with PCGrad to a list of methods mentioned in Appendix~\ref{app:sl_details}, where each method is trained with three different weighting schemes as in~\citep{liu2018attention}, equal weighting, weight uncertainty~\citep{kendall2017multi}, and DWA~\citep{liu2018attention}. We only run MTAN with PCGrad with weight uncertainty as we find weight uncertainty as the most effective scheme for training MTAN. The results comparing Cross-Stitch, MTAN and MTAN + PCGrad are presented in Table~\ref{tab:mtl_results_compare} while the full comparison can be found in Table~\ref{tab:nyu_results_full} in the Appendix~\ref{app:full_nyuv2_results}. MTAN with PCGrad is able to achieve the best scores in 8 out of the 9 categories where there are 3 categories per task.

Our multi-task supervised learning results indicate that PCGrad can be seamlessly combined with state-of-art multi-task learning architectures and further improve their results on established supervised multi-task learning benchmarks. We include more results of PCGrad combined with more multi-task learning architectures in Appendix~\ref{app:combined}.

\subsection{Multi-Task Reinforcement Learning}

\neurips{To answer question (2) in the RL setting}, \icml{we first consider the multi-task RL problem and evaluate our algorithm on the recently proposed Meta-World benchmark~\citep{metaworld}. In particular, we test all methods on the MT10 and MT50 benchmarks in Meta-World, which contain $10$ and $50$ manipulation tasks respectively shown in Figure~\ref{fig:metaworld}.} in Appendix~\ref{app:rl_details}.
%
%

%
%
%
%
%
%
%
%
%
%
%

\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\columnwidth]{figures/PCGrad_mt10_mt50_mag_dir_gradnorm.png}
    \vspace{-0.1cm}
    \caption{\footnotesize \neurips{For the two plots on the left, we show learning curves on MT10 and MT50 respectively. PCGrad significantly outperforms the other methods in terms of both success rates and data efficiency. In the rightmost plot, we present the ablation study on only using the magnitude and the direction of gradients modified by PCGrad and a comparison to GradNorm~\cite{chen2017gradnorm}. PCGrad outperforms both ablations and GradNorm, indicating the importance of modifying both the gradient directions and magnitudes in multi-task learning.}}
    \vspace{-0.2cm}
    \label{fig:rl_results}
\end{figure*}

The results are shown in left two plots in Figure~\ref{fig:rl_results}. PCGrad combined with SAC learns all tasks with the best data efficiency and successfully solves all of the $10$ tasks in MT10 and about $70$\% of the $50$ tasks in MT50. Training a single SAC policy and a multi-head policy is unable to acquire half of the skills in both MT10 and MT50, suggesting that eliminating gradient interference across tasks can significantly boost performance of multi-task RL. Training independent SAC agents is able to eventually solve all tasks in MT10 and $70$\% of the tasks in MT50, but requires about $2$ millions and $15$ millions more samples than PCGrad with SAC in MT10 and MT50 respectively, implying that applying PCGrad can result in leveraging shared structure among tasks that expedites multi-task learning.
As noted by~\citet{metaworld}, these tasks involve distinct behavior motions, which makes learning all tasks with a single policy challenging as demonstrated by poor baseline performance. The ability to learn these tasks together opens the door for a number of interesting extensions to meta-learning and generalization to novel task families. 
%

\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/theorem2_analysis.png}
    \caption{\footnotesize An empirical analysis of the theoretical conditions discussed in Theorem~\ref{thm:local}, showing the first $100$ iterations of training on two RL tasks, reach and press button top. \textbf{Left}: The estimated value of the multi-task curvature. We observe high multi-task curvatures exist throughout training, providing evidence for condition (b) in Theorem~\ref{thm:local}. \textbf{Middle}: The solid lines show the percentage gradients with positive cosine similarity between two task gradients, while the dotted lines and dashed lines show the percentage of iterations in which condition (a) and the implication of condition (b) ($\xi(\rvgone, \rvgtwo) \leq 1$) in Theorem~\ref{thm:local} are held respectively, among iterations when the cosine similarity is negative. \textbf{Right}: The average return of each task achieved by SAC and SAC combined with PCGrad. From the plots in the \textbf{Middle} and on the \textbf{Right}, we can tell that condition (a) holds most of the time for both Adam and Adam combined with PCGrad when they haven't solved Task 2 and as soon as Adam combined PCGrad starts to learn Task 2, the percentage of condition (a) held starts to decline. This observation suggests that condition (a) is a key factor for PCGrad excelling in multi-task learning.
    }
    \vspace{-0.3cm}
    \label{fig:analysis}
\end{figure*}

%
\neurips{Since the PCGrad update affects both the gradient direction and the gradient magnitude, we perform an ablation study that tests two variants of PCGrad: (1) only applying the gradient direction corrected with PCGrad while keeping the gradient magnitude unchanged and (2) only applying the gradient magnitude computed by PCGrad while keeping the gradient direction unchanged. We further run a direction comparison to GradNorm~\citep{chen2017gradnorm}, which also scales only the magnitudes of the task gradients.
%
As shown in the rightmost plot in Figure~\ref{fig:rl_results}, both variants and GradNorm perform worse than PCGrad and the variant where we only vary the gradient magnitude is much worse than PCGrad. This emphasizes the importance of the orientation change, which is particularly notable as multiple prior works only alter gradient magnitudes~\cite{chen2017gradnorm,sener2018multi}. We also notice that the variant of PCGrad where only the gradient magnitudes change achieves comparable performance to GradNorm, which suggests that it is important to modify both the gradient directions and magnitudes to eliminate interference and achieve good multi-task learning results. Finally, to test the importance of keeping positive cosine similarities between tasks for positive transfer, we compare PCGrad to a recently proposed method in~\cite{suteu2019regularizing} that regularizes cosine similarities of different task gradients towards $0$. PCGrad outperforms \citet{suteu2019regularizing} by a large margin. We leave details of the comparison to Appendix~\ref{app:cosine}}.
%

%

%

%
%
%
%
%
%
%
%

%
%

%

\subsection{Empirical Analysis of the Tragic Triad}
\label{sec:analysis}



Finally, to answer question (1), we \icmllast{compare the performance of standard multi-task SAC and the multi-task SAC with PCGrad. We evaluate each method on two tasks, reach and press button top, in the Meta-World~\cite{metaworld} benchmark.} As shown in the leftmost plot in Figure~\ref{fig:analysis}, we plot the multi-task curvature, which is computed as 
$
  \mathbf{H}(\mathcal{L};\theta^t\!,\! \theta^{t+1}\!)\! =\! 2\!\cdot\!\left[\mathcal{L}(\theta^{t+1})\!\!-\!\!\mathcal{L}(\theta^{t})\!\!-\!\! \nabla_{\theta^{t}}\mathcal{L}(\theta^{t})^T\!(\theta^{t+1}\!\!-\!\theta^{t})\right]
$
by Taylor's Theorem where $\mathcal{L}$ is the multi-task loss, and $\theta^{t}$ and $\theta^{t+1}$ are the parameters at iteration $t$ and $t+1$. During the training process, the multi-task curvature stays positive and is increasing for both Adam and Adam combined PCGrad, suggesting that condition (b) in Theorem~\ref{thm:local} that the multi-task curvature is lower bounded by some positive value is widely held empirically. 
%
\icml{To further analyze conditions in Theorem~\ref{thm:local} empirically, we plot the percentage of condition (a) (i.e. conflicting gradients) and the implication of condition (b) ($\xi(\rvgone, \rvgtwo) \leq 1$) in Theorem~\ref{thm:local} being held among the total number of iterations where the cosine similarity is negative in the plot in the middle of Figure~\ref{fig:analysis}. Along with the plot on the right in Figure~\ref{fig:analysis}, which presents the average return of the two tasks during training, we can see that while Adam and Adam with PCGrad haven't received reward signal from Task 2, condition (a) and the implication of condition (b) stay held and as soon as Adam with PCGrad begins to solve Task 2, the percentage of condition (a) and the implication of condition (b) being held start to decrease. Such a pattern suggests that conflicting gradients, high curvatures and dominating gradients indeed produce considerable challenges in optimization before multi-task learner gains any useful learning signal,  which also implies that the tragic triad may indeed be the determining factor where PCGrad can lead to better performance gain over standard multi-task learning in practice.}



==> Gradient Surgery for Multi-Task Learning NeurIPS/intro.tex <==
\section{Introduction}

While deep learning and deep reinforcement learning (RL) have shown considerable promise in enabling systems to learn complex tasks, the data requirements of current methods make it difficult to learn a breadth of capabilities, particularly when all tasks are learned individually from scratch. A natural approach to such multi-task learning problems is to train a network on all tasks jointly, with the aim of discovering shared structure across the tasks in a way that achieves greater efficiency and performance than solving tasks individually. However, learning multiple tasks all at once results is a difficult optimization problem, sometimes leading to \emph{worse} overall performance and data efficiency compared to learning tasks individually~\citep{parisotto2015actor,rusu2015policydistillation}. These optimization challenges are so prevalent that multiple multi-task RL algorithms have considered using independent training as a subroutine of the algorithm before distilling the independent models into a multi-tasking model~\citep{levine2016end,parisotto2015actor,rusu2015policydistillation,ghosh2017dnc,teh2017distral}, producing a multi-task model but losing out on the efficiency gains over independent training. If we could tackle the optimization challenges of multi-task learning effectively, we may be able to actually realize the hypothesized benefits of multi-task learning without the cost in final performance.

\begin{wrapfigure}{R}{0.59\textwidth}
%
    \centering
    \includegraphics[width=1.0\linewidth]{figures/pcgrad_example.png}
    \vspace{-0.4cm}
    \caption{\footnotesize Visualization of \arxiv{PCGrad} on a 2D multi-task optimization problem. (a) A multi-task objective landscape. (b) \& (c) Contour plots of the individual task objectives that comprise (a). (d) Trajectory of gradient updates on the multi-task objective using the Adam optimizer. The gradient vectors of the two tasks at the end of the trajectory are indicated by blue and red arrows, where the relative lengths are on a log scale.(e) Trajectory of gradient updates on the multi-task objective using Adam with PCGrad. For (d) and (e), the optimization trajectory goes from black to yellow.}
    \vspace{-0.3cm}
    \label{fig:optlandscape}
%
\end{wrapfigure}

While there has been a significant amount of research in multi-task learning~\citep{caruana97multitask,ruder2017overview}, the optimization challenges are not well understood. Prior work has described varying learning speeds of different tasks~\citep{chen2017gradnorm,hessel2019popart} and \arxiv{plateaus} in the optimization landscape~\citep{schaul2019ray} as potential causes, whereas a range of other works have focused on the model architecture~\citep{misra2016crossstitch,liu2018attention}. In this work, we instead hypothesize that one of the main optimization issues in multi-task learning arises from gradients from different tasks conflicting with one another in a way that is detrimental to making progress. We define two gradients to be conflicting if they point away from one another, i.e., have a negative cosine similarity. We hypothesize that such conflict is detrimental when a) conflicting gradients coincide with b) high positive curvature and c) a large difference in gradient magnitudes.

As an illustrative example, consider the 2D optimization landscapes of two task objectives in Figure~\ref{fig:optlandscape}a-c.
\icml{The optimization landscape of each task consists of a deep valley, a property that has been observed in neural network optimization landscapes~\citep{goodfellow2014qualitatively}, and the bottom of each valley is characterized by high positive curvature and large differences in the task gradient magnitudes.
%
Under such circumstances, the multi-task gradient is dominated by one task gradient, which comes at the cost of degrading the performance of the other task. Further, due to high curvature, the improvement in the dominating task may be overestimated, while the degradation in performance of the non-dominating task may be underestimated.
As a result, the optimizer struggles to make progress on the optimization objective. In Figure~\ref{fig:optlandscape}d), the optimizer reaches the deep valley of task 1, but is unable to traverse the valley in a parameter setting where there are \icmllast{\emph{conflicting gradients}, \emph{high curvature}, and \emph{a large difference in gradient magnitudes}} (see gradients plotted in Fig.~\ref{fig:optlandscape}d).
In Section~\ref{sec:analysis}, we find experimentally that this \emph{tragic triad}
also occurs in a higher-dimensional neural network multi-task learning problem.}

The core contribution of this work is a method for mitigating gradient interference by altering the gradients directly, i.e. by performing ``gradient surgery.'' If two gradients are conflicting, we alter the gradients by projecting each onto the normal plane of the other, preventing the interfering components of the gradient from being applied to the network. We refer to this particular form of gradient surgery as \emph{projecting conflicting gradients} (PCGrad). PCGrad is model-agnostic, requiring only a single modification to the application of gradients. Hence, it is easy to apply to a range of problem settings, including multi-task supervised learning
and multi-task reinforcement learning, and can also be readily combined with other multi-task learning approaches, such as those that modify the architecture. \icml{We theoretically prove the local conditions under which PCGrad improves upon standard multi-task gradient descent}, and we empirically evaluate PCGrad on a variety of challenging problems, including multi-task CIFAR classification, multi-objective scene understanding, a challenging multi-task RL domain, and goal-conditioned RL. Across the board, we find PCGrad leads to substantial improvements in terms of data efficiency, optimization speed, and final performance compared to prior approaches, including a more than 30\% absolute improvement in multi-task reinforcement  learning problems. Further, on multi-task supervised learning tasks, PCGrad can be successfully combined with prior state-of-the-art methods for multi-task learning for even greater performance. 




%



==> Gradient Surgery for Multi-Task Learning NeurIPS/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}
\usepackage{amsthm, amssymb, bbm}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{mathtools}

% Math
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{corollary}{Corollary}
\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
\newtheorem{notation}{Notation}
\newtheorem{obs}{Observation}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Gradient Surgery for Multi-Task Learning NeurIPS/method.tex <==
\def\rvgone{{\mathbf{g}_1}}
\def\rvgtwo{{\mathbf{g}_2}}
\def\rvg{{\mathbf{g}}}

\section{Multi-Task Learning with PCGrad}

\newcommand{\btheta}{\bm \theta}

While the multi-task problem can in principle be solved by simply applying a standard single-task algorithm with a suitable task identifier provided to the model, or a simple multi-head or multi-output model, a number of prior works~\citep{parisotto2015actor,rusu2015policydistillation,sener2018multi} have found this learning problem to be difficult. %
%
In this section, we introduce notation, identify possible causes for the difficulty of multi-task optimization, propose a simple and general approach to mitigate it, and theoretically analyze the proposed approach. 

\input{prelim.tex}

\subsection{\!\!\!The Tragic Triad: Conflicting Gradients, Dominating Gradients, High Curvature}
\label{sec:tragictriad}

\icml{We hypothesize that a key optimization issue in multi-task learning arises from conflicting gradients, where gradients for different tasks point away from one another as measured by a negative inner product. However, conflicting gradients are not detrimental on their own. Indeed, simply averaging task gradients should provide the correct solution to descend the multi-task objective. However, there are conditions under which such conflicting gradients lead to significantly degraded performance. Consider a two-task optimization problem. If the gradient of one task is much larger in magnitude than the other, it will dominate the average gradient. %
If there is also high positive curvature along the directions of the task gradients, then the improvement in performance from the dominating task may be significantly overestimated, while the degradation in performance from the dominated task may be significantly underestimated.
Hence, we can characterize the co-occurrence of three conditions as follows: (a) when gradients from multiple tasks are in conflict with one another (b) when the difference in gradient magnitudes is large, leading to some task gradients dominating others, and (c) when there is high curvature in the multi-task optimization landscape. We formally define the three conditions below.}

\begin{definition}
\label{def:angle}
We define $\phi_{ij}$ as the angle between two task gradients $\mathbf{g}_i$ and $\mathbf{g}_j$. We define the gradients as \textbf{conflicting} when $\cos\phi_{ij}<0$.
\end{definition}

\begin{definition}
\label{def:div}
We define the \textbf{gradient magnitude similarity} between two gradients $\mathbf{g}_i$ and $\mathbf{g}_j$
as 
$
    \Phi(\mathbf{g}_i, \mathbf{g}_j) = \frac{2\|\mathbf{g}_i\|_2\|\mathbf{g}_j\|_2}{\|\mathbf{g}_i\|_2^2 + \|\mathbf{g}_j\|_2^2}.
$
\end{definition}
When the magnitude of two gradients is the same, this value is equal to 1. As the gradient magnitudes become increasingly different, this value goes to zero.

\begin{definition}
\label{def:curvature}
We define \textbf{multi-task curvature} as 
$
    \mathbf{H}(\loss; \theta, \theta') = \int_0^1\nabla\loss(\theta)^T\nabla^2\loss(\theta + a(\theta'-\theta))\nabla\loss(\theta)da,
$
which is the averaged curvature of $\loss$ between $\theta$ and $\theta'$ in the direction of the multi-task gradient $\nabla\loss(\theta)$.
\end{definition}

When $\mathbf{H}(\loss; \theta, \theta') > C$ for some large positive constant $C$, for model parameters $\theta$ and $\theta'$ at the current and next iteration, we characterize the optimization landscape as having high curvature.

%

%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

\icml{We aim to study the tragic triad and observe the presence of the three conditions through two examples. First, consider the two-dimensional optimization landscape illustrated in Fig.~\ref{fig:optlandscape}a, where the landscape for each task objective corresponds to a deep and curved valley with large curvatures (Fig.~\ref{fig:optlandscape}b and~\ref{fig:optlandscape}c). The optima of this multi-task objective correspond to where the two valleys meet. More details on the optimization landscape are in Appendix~\ref{app:optimization_landscape_details}. Particular points of this optimization landscape exhibit the three described conditions, and we observe that, the Adam~\citep{kingma2014adam} optimizer stalls precisely at one of these points (see Fig.~\ref{fig:optlandscape}d), preventing it from reaching an optimum. This provides some empirical evidence for our hypothesis. Our experiments in Section~\ref{sec:analysis} further suggest that this phenomenon occurs in multi-task learning with deep networks.
Motivated by these observations, we develop an algorithm that aims to alleviate the optimization challenges caused by conflicting gradients, dominating gradients, and high curvature, which we describe next.}

\iffalse
\icml{We also aim to detect if a similar phenomenon occurs in multi-task learning with a neural network on the multi-task CIFAR-100 domain (see Section~\ref{sec:experiments} for details).
\KH{To analyze the extent of these three conditions, we measure the occurrence of conflicting gradients, the occurrence of dominating gradients, and the estimated curvature along the direction of the multi-task gradient.}
%
We indeed observe a significant occurrence of these three conditions when training deep neural networks on multi-task problems --- the percentage of the conflicting gradients is at least 38\%, a gradient dominates XX\% of the time, and the curvature along the gradient remains positive throughout training.}
\todo{Kevin -- fill in the above statistic about dominating gradients, in a way that makes sense}
\fi



\subsection{\!\!\!PCGrad: Project Conflicting Gradients}\label{sec:pcgrad}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\batch}{\mathcal{B}}

Our goal is to break one condition of \icml{the tragic triad} by directly altering the gradients themselves to prevent conflict. In this section, we outline our approach for altering the gradients. \icml{In the next section, we will theoretically show that de-conflicting gradients can benefit multi-task learning when dominating gradients and high curvatures are present}.

To be maximally effective and widely applicable, we aim to alter the gradients in a way that allows for positive interactions between the task gradients and does not introduce assumptions on the form of the model. Hence, when gradients do not conflict, we do not change the gradients.
%
When gradients do conflict, the goal of PCGrad is to modify the gradients for each task so as to minimize negative conflict with other task gradients, which will in turn mitigate under- and over-estimation problems arising from \icml{high curvature}.
%
%

To deconflict gradients during optimization, PCGrad adopts a simple procedure: if the gradients between two tasks are in conflict, i.e. their cosine similarity is negative, we project the gradient of each task onto the normal plane of the gradient of the other task. 
This amounts to removing the conflicting component of the gradient for the task, thereby reducing the amount of destructive gradient interference between tasks. 
A pictorial description of this idea is shown in Fig.~\ref{fig:conflict}.
\begin{minipage}[t]{\linewidth}
\centering
      \begin{minipage}[t]{0.495\linewidth}
          \begin{algorithm}[H]
            \caption{ PCGrad Update Rule}
            \label{alg:dgrad-o}
            \begin{algorithmic}[1]
            {\small
            %
            \REQUIRE Model parameters $\theta$, task minibatch $\batch =\{\task_k\}$
            %
            \STATE $\bg_k \leftarrow \nabla_\theta \loss_k(\theta) ~~\forall k$
            \STATE $\bg_k^{\text{PC}} \leftarrow \bg_k ~~\forall k$
            \FOR{$\task_i \in \batch$ } %
                %
                \FOR{$\task_j \stackrel{\text{\scriptsize uniformly}}{\sim} \batch \setminus \task_i$ \arxiv{in random order}}
                      %
                      %
                    %
                      \IF{$\bg_i^{\text{PC}} \cdot \bg_j < 0$}
                      %
                        \STATE \textit{// Subtract the projection of} $\bg_i^{\text{PC}}$ \textit{onto} $\bg_j$
                        \STATE Set $\bg_i^{\text{PC}} = \bg_i^{\text{PC}} - \frac{\bg_i^{\text{PC}} \cdot \bg_j}{\|\bg_j\|^2} \bg_j $ 
                      \ENDIF
                \ENDFOR
                %
             \ENDFOR
            \STATE \textbf{return} update $\Delta \theta = \bg^\text{PC} = \sum_i \bg_i^{\text{PC}}$
            }
            \end{algorithmic}
            \end{algorithm}
            \vspace{-0.1cm}
      \end{minipage}
    %
      \begin{minipage}[t]{0.495\linewidth}
          \begin{figure}[H]
              \includegraphics[width=0.99\linewidth]{figures/grads.png}
              \vspace{-0.5cm}
              \captionof{figure}{\footnotesize Conflicting gradients and PCGrad. In (a), tasks $i$ and $j$ have conflicting gradient directions, which can lead to destructive interference. In (b) and (c), we illustrate the PCGrad algorithm in the case where gradients are conflicting. PCGrad projects task $i$'s gradient onto the normal vector of task $j$'s gradient, and vice versa. Non-conflicting task gradients (d) are not altered under PCGrad, allowing for constructive interaction.}
              \label{fig:conflict}
          \end{figure}
      \end{minipage}
\end{minipage}
Suppose the gradient for task $\task_i$ is $\bg_i$, and the gradient for task $\task_j$ is $\bg_j$. PCGrad proceeds as follows: (1) First, it determines whether $\bg_i$ conflicts with $\bg_j$ by computing the cosine similarity between vectors $\bg_i$ and $\bg_j$, where negative values indicate conflicting gradients. (2) If the cosine similarity is negative, we replace $\bg_i$ by its projection onto the normal plane of $\bg_j$: $\bg_i = \bg_i - \frac{\bg_i \cdot \bg_j}{\|\bg_j\|^2}\bg_j$. 
If the gradients are not in conflict, i.e. cosine similarity is non-negative, the original gradient $\bg_i$ remains unaltered. (3) PCGrad repeats this process across all of the other tasks sampled \arxiv{in random order from} the current batch $\task_j~ \forall~j\neq i$, resulting in the gradient $\bg_i^{\text{PC}}$ that is applied for task $\task_i$.
We perform the same procedure for all tasks in the batch to obtain their respective gradients. 
The full update procedure is described in Algorithm~\ref{alg:dgrad-o} \arxiv{and a discussion on using a random task order is included in Appendix~\ref{app:ablation_order}}.
%
%
%
%
%
%
%
%
%
%
%

\iffalse
, and can also be expressed as a single equation as follows:
\begin{align}
\Delta \theta = \sum_{\task_i\in\batch} \left[ \bg_i - \sum_{\task_j\in\batch}  \mathbbm{1}(\cos(\theta_{ij})<0) \frac{\bg_i\cdot\bg_j}{\|\bg_i\|^2}\bg_j    \right]\\
\text{where } ~~~ \bg_k = \nabla_\theta \loss_k(\theta), ~~~~~ \cos(\theta_{ij}) = \frac{\bg_i \cdot \bg_j}{\|\bg_j\|\|\bg_j\|} \nonumber
\end{align}
and where $\batch$ corresponds to a minibatch of tasks sampled from $p(\task)$ and where the PCGrad update $\Delta \theta$ can be plugged into SGD algorithms such as momentum and Adam without modification.
\fi


This procedure, while simple to implement, ensures that the gradients that we apply for each task per batch interfere minimally with the other tasks in the batch, mitigating the \icml{conflicting gradient} problem, producing a variant on standard first-order gradient descent in the multi-objective setting. In practice,  PCGrad can be combined with any gradient-based optimizer, including commonly used methods such as SGD with momentum and Adam~\citep{kingma2014adam}, by simply passing the computed update to the respective optimizer instead of the original gradient. Our experimental results verify the hypothesis that this procedure reduces the problem of \icml{conflicting gradients}, and find that, as a result, learning progress is substantially improved.




\subsection{Theoretical Analysis of PCGrad}
\label{sec:theory}

\icml{
In this section, we theoretically analyze the performance of PCGrad with two tasks:
\begin{definition}
\label{def:setup}
Consider two task loss functions $\loss_1 : \mathbb{R}^n \rightarrow \mathbb{R}$ and $\loss_2 : \mathbb{R}^n \rightarrow \mathbb{R}$. We define the two-task learning objective as $\loss(\theta) = \loss_1(\theta) + \loss_2(\theta)$ for all $\theta \in \mathbb{R}^n$, where $\rvgone = \nabla \loss_1(\theta)$, $\rvgtwo = \nabla \loss_2(\theta)$, and $\rvg = \rvgone + \rvgtwo$.
\end{definition}
}

We first aim to verify that the PCGrad update corresponds to a sensible optimization procedure under simplifying assumptions. We analyze convergence of PCGrad in the convex setting, under standard assumptions in Theorem~\ref{thm:converge}.
%
\neurips{For additional analysis on convergence, including the non-convex setting, with more than two tasks, and with momentum-based optimizers, see Appendices~\ref{app:proof} and \ref{app:momentum}}
%
%
\begin{restatable}{theorem}{theoremconvergence}
\label{thm:converge}
Assume $\loss_1$ and $\loss_2$ are convex and differentiable.
Suppose the gradient of $\loss$ is $L$-Lipschitz with $L > 0$.
%
Then, the PCGrad update rule with step size $t \leq \frac{1}{L}$ will converge to either (1) a location in the optimization landscape where $\cos(\phi_{12}) = -1$ or (2) the optimal value $\loss(\theta^*)$.
\end{restatable}

\vspace{-0.3cm}
\begin{proof}
See Appendix~\ref{app:proof}.
\end{proof}
\vspace{-0.3cm}

Theorem~\ref{thm:converge} states that application of the PCGrad update in the two-task setting with a convex and Lipschitz multi-task loss function $\loss$ leads to convergence to either the minimizer of $\loss$ or a potentially sub-optimal objective value. A sub-optimal solution occurs when the cosine similarity between the gradients of the two tasks is exactly $-1$, i.e. the gradients directly conflict, leading to zero gradient after applying PCGrad. However, in practice, since we are using SGD, which is a noisy estimate of the true batch gradients, the cosine similarity between the gradients of two tasks in a minibatch is unlikely to be $-1$, thus avoiding this scenario. 
%
%
\neurips{Note that, in theory, convergence may be slow if $\cos(\phi_{12})$ hovers near $-1$. However, we don't observe this in practice, as seen in the objective-wise learning curves in Appendix~\ref{app:objective-wise}.}


Now that we have checked the sensibility of PCGrad, we aim to understand how PCGrad relates to the three conditions in the tragic triad. In particular, we derive sufficient conditions under which PCGrad achieves lower loss after one update. Here, we still analyze the two task setting, but no longer assume convexity of the loss functions.

\begin{definition}
\label{def:bounding}
\icml{We define the \textbf{multi-task curvature bounding measure}
$\xi(\rvgone, \rvgtwo) = (1 - \cos^2\phi_{12})\frac{\|\rvgone-\rvgtwo\|_2^2}{\|\rvgone + \rvgtwo\|_2^2}.$}
\end{definition}
With the above definition, we present our next theorem:
\begin{restatable}{theorem}{theoremlocal}
\label{thm:local}
Suppose $\loss$ is differentiable and the gradient of $\loss$ is Lipschitz continuous with constant $L > 0$. 
Let $\theta^{\text{MT}}$ and $\theta^{\text{PCGrad}}$ be the parameters after applying one update to $\theta$ with $\rvg$ and PCGrad-modified gradient $\rvg^{\text{PC}}$ respectively, with step size $t > 0$. 
Moreover, assume $\mathbf{H}(\loss; \theta, \theta^{\text{MT}}) \geq \ell\|\rvg\|_2^2$ for some constant $\ell \leq L$, i.e. the multi-task curvature is lower-bounded.
Then $\loss(\theta^{\text{PCGrad}}) \leq \loss(\theta^{\text{MT}})$ if \textbf{(a)} $\cos\phi_{12} \leq -\Phi(\rvgone, \rvgtwo)$, \textbf{(b)} $\ell \geq \xi(\rvgone, \rvgtwo)L$, and \textbf{(c)} $t \geq \frac{2}{\ell - \xi(\rvgone, \rvgtwo)L}.$
%
%
%
%
%
%
%
%
%
%
\end{restatable}

\vspace{-0.3cm}
\begin{proof}
See Appendix~\ref{app:proof2}.
\end{proof}
\vspace{-0.3cm}

%
\icml{Intuitively, Theorem~\ref{thm:local} implies that PCGrad achieves lower loss value after a single gradient update compared to standard gradient descent in multi-task learning when (i) the angle between task gradients is not too small, i.e. the two tasks need to conflict sufficiently (\textbf{condition (a)}), (ii) the difference in magnitude needs to be sufficiently large (\textbf{condition (a)}), (iii) the curvature of the multi-task gradient should be large (\textbf{condition (b)}), (iv) and the learning rate should be big enough so that large curvature would lead to overestimation of performance improvement on the dominating task and underestimation of performance degradation on the dominated task (\textbf{condition (c)}). These first three points (i-iii) correspond to exactly the triad of conditions outlined in Section~\ref{sec:tragictriad}, while the latter condition (iv) is desirable as we hope to learn quickly. We empirically validate that the first three points, (i-iii), are frequently met in a neural network multi-task learning problem in Figure~\ref{fig:analysis} in Section~\ref{sec:analysis}.} \neurips{For additional analysis, including complete sufficient and necessary conditions for the PCGrad update to outperform the vanilla multi-task gradient, see Appendix~\ref{app:theorem3}.}
%
%



\section{PCGrad in Practice}
\label{sec:pcgrad_practical}

We use PCGrad in supervised learning and reinforcement learning problems with multiple tasks or goals. Here, we discuss the practical application of PCGrad to those settings. %

In multi-task supervised learning, each task $\task_i \sim p(\task)$ has a corresponding training dataset $\mathcal{D}_i$ consisting of labeled training examples, i.e. $\mathcal{D}_i = \{(x, y)_n\}$. 
The objective for each task in this supervised setting is then defined as $\loss_i(\theta) = \mathbb{E}_{(x,y) \sim \data_i} \left[ - \log f_\theta(y | x, z_i ) \right]$, where $z_i$ is a one-hot encoding of task $\task_i$. 
At each training step, we randomly sample a batch of data points $\mathcal{B}$ from the whole dataset $\bigcup_i \mathcal{D}_i$ and then group the sampled data with the same task encoding into small batches denoted as $\mathcal{B}_{i}$ for each $\task_i$ represented in $\mathcal{B}$. We denote the set of tasks appearing in $\mathcal{B}$ as $\mathcal{B}_\task$. After sampling, we precompute the gradient of each task in $\mathcal{B}_\task$ as
$
    \nabla_\theta \mathcal{L}_i(\theta) = \mathbb{E}_{(x,y) \sim \mathcal{B}_i} \left[ - \nabla_\theta\log f_\theta(y | x, z_i ) \right]\text{.}
$
Given the set of precomputed gradients $\nabla_\theta \mathcal{L}_i(\theta)$, we also precompute the cosine similarity between all pairs of the gradients in the set. Using the pre-computed gradients and their similarities, we can obtain the PCGrad  update by following Algorithm~\ref{alg:dgrad-o}, without re-computing task gradients nor backpropagating into the network.
Since the PCGrad procedure is only modifying the gradients of shared parameters in the optimization step, it is \textit{model-agnostic} and can be applied to any architecture with shared parameters.
%
\neurips{We empirically validate PCGrad with multiple architectures in Section~\ref{sec:experiments}}.

\icml{For multi-task RL and goal-conditioned RL, PCGrad can be readily applied to policy gradient methods by directly updating the computed policy gradient of each task, following Algorithm~\ref{alg:dgrad-o}, analogous to the supervised learning setting. For actor-critic algorithms, it is also straightforward to apply PCGrad: we simply replace task gradients for both the actor and the critic by their gradients computed via PCGrad.} \neurips{For more details on the practical implementation for RL, see Appendix~\ref{app:practical_rl}.}
%


%
%




==> Gradient Surgery for Multi-Task Learning NeurIPS/prelim.tex <==
\subsection{Preliminaries: Problem and Notation}
\label{sec:prelim}


\newcommand{\task}{\mathcal{T}}
%
%

The goal of multi-task learning is to find parameters $\theta$ of a model $f_\theta$ that achieve high average performance across all the training tasks drawn from a distribution of tasks $p(\task)$. 
More formally, we aim to solve the problem: $\min\limits_{\theta} \mathbb{E}_{\task_i \sim p(\task)} \left[ \mathcal{L}_i(\theta) \right]$, where $\mathcal{L}_i$ is a loss function for the $i$-th task $\task_i$ that we want to minimize. For a set of tasks, $\{\task_i\}$, we denote the multi-task loss as $\loss(\theta) = \sum_i \loss_i(\theta)$, and the gradients of each task as $\mathbf{g}_i = \nabla \loss_i(\theta)$ for a particular $\theta$. (We drop the reliance on $\theta$ in the notation for brevity.)
%
To obtain a model that solves a specific task from the task distribution $p(\task)$, we define a task-conditioned model $f_\theta(y|x, z_i)$, with input $x$, output $y$, and encoding $z_i$ for task $\task_i$, which could be provided as a one-hot vector or in any other form.


%

%
%

%

%
%
%
%
%
%


==> Gradient Surgery for Multi-Task Learning NeurIPS/proofs.tex <==
\def\rvgone{{\mathbf{g_1}}}
\def\rvgtwo{{\mathbf{g_2}}}



\section{Proofs}
\subsection{Proof of Theorem 1}
\label{app:proof}
\theoremconvergence*

\begin{proof}

We will use the shorthand $|| \cdot ||$ to denote the $L_2$-norm and $\nabla \loss = \nabla_\theta \loss$, where $\theta$ is the parameter vector. Following Definition~\ref{def:angle} and \ref{def:setup}, let $\rvgone = \nabla \loss_1$, $\rvgtwo = \nabla \loss_2$, $\rvg = \nabla\loss = \rvgone + \rvgtwo$, and $\phi_{12}$ be the angle between $\rvgone$ and $\rvgtwo$.

At each PCGrad update, we have two cases: $cos(\phi_{12}) \geq 0$ or $\cos(\phi_{12} ) < 0$.

If $\cos(\phi_{12}) \geq 0$, then we apply the standard gradient descent update using $t \leq \frac{1}{L}$, which leads to a strict decrease in the objective function value $\loss(\theta)$ (since it is also convex) unless $\nabla \loss(\theta) = 0$, which occurs only when $\theta = \theta^*$~\citep{boyd2004convex}. 

In the case that $\cos(\phi_{12}) < 0$, we proceed as follows:

Our assumption that $\nabla \loss$ is Lipschitz continuous with constant $L$ implies that $\nabla^2 \loss(\theta) - LI$ is a negative semi-definite matrix. Using this fact, we can perform a quadratic expansion of $\loss$ around $\loss(\theta)$ and obtain the following inequality:
\begin{align*}
\loss(\theta^+) &\leq \loss(\theta) + \nabla \loss(\theta)^T (\theta^+ - \theta) + \frac{1}{2} \nabla^2 \loss(\theta) ||\theta^+ - \theta||^2 \\
&\leq \loss(\theta) + \nabla \loss(\theta)^T (\theta^+ - \theta) + \frac{1}{2} L ||\theta^+ - \theta||^2
\end{align*}
Now, we can plug in the PCGrad update by letting $\theta^+ = \theta - t\cdot(\rvg - \frac{\rvgone \cdot \rvgtwo}{||\rvgone||^2}\rvgone - \frac{\rvgone \cdot \rvgtwo}{||\rvgtwo||^2}\rvgtwo)$. We then get:
\begin{align}
    \loss(\theta^+) &\leq \loss(\theta) + t\cdot\rvg^T (-\rvg + \frac{\rvgone \cdot \rvgtwo}{||\rvgone||^2}\rvgone + \frac{\rvgone \cdot \rvgtwo}{||\rvgtwo||^2}\rvgtwo) 
    + \frac{1}{2}Lt^2||\rvg - \frac{\rvgone \cdot \rvgtwo}{||\rvgone||^2}\rvgone - \frac{\rvgone \cdot \rvgtwo}{||\rvgtwo||^2}\rvgtwo||^2\nonumber \\ \nonumber\\
    &\text{(Expanding, using the identity $\rvg = \rvgone + \rvgtwo$)}\nonumber
    \\ \nonumber\\
    &= \loss(\theta) + t\left(-||\rvgone||^2 - ||\rvgtwo||^2 + \frac{(\rvgone \cdot \rvgtwo)^2}{||\rvgone||^2} + \frac{(\rvgone \cdot \rvgtwo)^2}{||\rvgtwo||^2}\right)
    + \frac{1}{2}Lt^2||\rvgone + \rvgtwo \nonumber\\ 
    &- \frac{\rvgone \cdot \rvgtwo}{||\rvgone||^2}\rvgone - \frac{\rvgone \cdot \rvgtwo}{||\rvgtwo||^2}\rvgtwo||^2\nonumber
    \\ \nonumber\\
    &\text{(Expanding further and re-arranging terms)}\nonumber
    \\ \nonumber\\
    &= \loss(\theta) - (t - \frac{1}{2}Lt^2)(||\rvgone||^2 + ||\rvgtwo||^2 - \frac{(\rvgone \cdot \rvgtwo)^2}{||\rvgone||^2} - \frac{(\rvgone \cdot \rvgtwo)^2}{||\rvgtwo||^2})\nonumber\\
    &- Lt^2(\rvgone \cdot \rvgtwo - \frac{(\rvgone \cdot \rvgtwo)^2}{||\rvgone||^2 ||\rvgtwo||^2}\rvgone \cdot \rvgtwo) \nonumber
    \\ \nonumber\\
    &\text{(Using the identity $\cos(\phi_{12}) = \frac{\rvgone \cdot \rvgtwo}{||\rvgone|| ||\rvgtwo||}$)}\nonumber
    \\ \nonumber\\
    &= \loss(\theta) - (t  - \frac{1}{2}Lt^2) [(1 - \cos^2(\phi_{12})) ||\rvgone||^2 + (1 - \cos^2(\phi_{12})) ||\rvgtwo||^2 ]\nonumber \\
    &- Lt^2 (1 - \cos^2(\phi_{12})) ||\rvgone|| ||\rvgtwo|| \cos(\phi_{12}) \label{eq:pcgrad_bound}\\
    &\text{(Note that $\cos(\phi_{12}) < 0$ so the final term is non-negative)}\nonumber
\end{align}
Using $t \leq \frac{1}{L}$, we know that $-(1 - \frac{1}{2} Lt) = \frac{1}{2}Lt - 1 \leq \frac{1}{2}L(1/L) - 1 = \frac{-1}{2}$ and $Lt^2 \leq t$. 

Plugging this into the last expression above, we can conclude the following:
\begin{align*}
    \loss(\theta^+) &\leq \loss(\theta) - \frac{1}{2}t [(1 - \cos^2(\phi_{12})) ||\rvgone||^2 + (1 - \cos^2(\phi_{12})) ||\rvgtwo||^2 ]\\
    &- t (1 - \cos^2(\phi_{12})) ||\rvgone|| ||\rvgtwo|| \cos(\phi_{12}) \\
    &= \loss(\theta) - \frac{1}{2}t (1 - \cos^2(\phi_{12})) [ ||\rvgone||^2 + 
    2 ||\rvgone|| ||\rvgtwo|| \cos(\phi_{12}) +
    ||\rvgtwo||^2 ] \\
    &= \loss(\theta) - \frac{1}{2}t (1 - \cos^2(\phi_{12})) [ ||\rvgone||^2 + 
    2 \rvgone \cdot \rvgtwo +
    ||\rvgtwo||^2 ] \\
    &= \loss(\theta) - \frac{1}{2}t (1 - \cos^2(\phi_{12})) ||\rvgone + \rvgtwo||^2 \\
    &= \loss(\theta) - \frac{1}{2}t (1 - \cos^2(\phi_{12})) \|\rvg\|^2
\end{align*}

If $\cos(\phi_{12}) > -1$, then $\frac{1}{2}t (1 - \cos^2(\phi_{12})) \|\rvg\|^2$ will always be positive unless $\rvg = 0$. This inequality implies that the objective function
value strictly decreases with each iteration where $\cos(\phi_{12}) > -1$.

Hence repeatedly applying PCGrad process can either reach the optimal value $\loss(\theta) = \loss(\theta^*)$ or $\cos(\phi_{12}) = -1$, in which case $\frac{1}{2}t (1 - \cos^2(\phi_{12})) \|\rvg\|^2 = 0$. Note that this result only holds when we choose $t$ to be small enough, i.e. $t \leq \frac{1}{L}$.

\end{proof}

\begin{corollary}
\label{cor:moretasks}
Assume the $n$ objectives $\loss_1, \loss_2, ..., \loss_n$ are convex and differentiable. Suppose the gradient of $\loss$ is Lipschitz continuous with constant $L > 0$. Assume that $\cos(\rvg, \rvg^\text{PC}) \geq \frac{1}{2}$. 
Then, the PCGrad update rule with step size $t \leq \frac{1}{L}$ will converge to either (1) a location in the optimization landscape where $\cos(\rvg_i, \rvg_j) = -1 \forall i, j$ or (2) the optimal value $\loss(\theta^*)$. 
\end{corollary}
\begin{proof}
Our assumption that $\nabla \loss$ is Lipschitz continuous with constant $L$ implies that $\nabla^2 \loss(\theta) - LI$ is a negative semi-definite matrix. Using this fact, we can perform a quadratic expansion of $\loss$ around $\loss(\theta)$ and obtain the following inequality:
\begin{align*}
\loss(\theta^+) &\leq \loss(\theta) + \nabla \loss(\theta)^T (\theta^+ - \theta) + \frac{1}{2} \nabla^2 \loss(\theta) ||\theta^+ - \theta||^2 \\
&\leq \loss(\theta) + \nabla \loss(\theta)^T (\theta^+ - \theta) + \frac{1}{2} L ||\theta^+ - \theta||^2
\end{align*}
Now, we can plug in the PCGrad update by letting $\theta^+ = \theta - t\cdot \rvg^\text{PC}$. We then get:
\begin{align*}
    \loss(\theta^+) &\leq \loss(\theta) - t\cdot\rvg^T \rvg^\text{PC}
    + \frac{1}{2}Lt^2||\rvg^\text{PC}||^2\nonumber \\
    &\text{(Using the assumption that $\cos(\rvg, \rvg^\text{PC}) \geq \frac{1}{2}$.)} \\
    &\leq \loss(\theta) - \frac{1}{2} t||\rvg||\cdot||\rvg^\text{PC}||
    + \frac{1}{2}Lt^2||\rvg^\text{PC}||^2\nonumber \\
    &\leq \loss(\theta) - \frac{1}{2} t||\rvg||\cdot||\rvg^\text{PC}||
    + \frac{1}{2}Lt^2||\rvg^\text{PC}|| \cdot ||\rvg|| \nonumber \nonumber \\
\end{align*}
Note that $-\frac{1}{2} t ||\rvg||\cdot||\rvg^\text{PC}||
    + \frac{1}{2}Lt^2||\rvg^\text{PC}|| \cdot ||\rvg|| \leq 0$ when $t \leq \frac{1}{L}$. Further, when $t < \frac{1}{L}$, $-\frac{1}{2} t ||\rvg||\cdot||\rvg^\text{PC}||
    + \frac{1}{2}Lt^2||\rvg^\text{PC}|| \cdot ||\rvg|| = 0$ if and only if $||\rvg|| = 0$ or $||\rvg^\text{PC}||=0$. 
    
Hence repeatedly applying PCGrad process can either reach the optimal value $\loss(\theta) = \loss(\theta^*)$ or a location in the optimization landscape where $\cos(\rvg_i, \rvg_j) = -1$ for all pairs of tasks $i, j$. Note that this result only holds when we choose $t$ to be small enough, i.e. $t \leq \frac{1}{L}$.
\end{proof}

\begin{proposition}
\label{prop:nonconvex}
Assume $\loss_1$ and $\loss_2$ are differentiable but possibly non-convex. Suppose the gradient of $\loss$ is Lipschitz continuous with constant $L > 0$.
Then, the PCGrad update rule with step size $t \leq \frac{1}{L}$ will converge to either (1) a location in the optimization landscape where $\cos(\phi_{12}) = -1$ or (2) find a $\theta_k$ that is almost a stationary point.
\end{proposition}
\begin{proof}
Following Definition~\ref{def:angle} and \ref{def:setup}, let $\rvgone_k = \nabla \loss_1$ at iteration $k$, $\rvgtwo_k = \nabla \loss_2$ at iteration $k$, and $\rvg_k = \nabla\loss = \rvgone_k + \rvgtwo_k$ at iteration $k$, and $\phi_{12, k}$ be the angle between $\rvgone_k$ and $\rvgtwo_k$.


From the proof of Theorem 1, when $\cos(\phi_{12},k) < 0$ we have:
$$
||\rvg_k||^2 \leq \frac{2}{t} \frac{\loss(\theta_{k-1}) - \loss(\theta_{k})}{(1 - \cos^2(\phi_{12, k}))}.
$$

Thus, we have:
\begin{align*}
\min_{0 \leq k \leq K} || \rvg_k ||^2 &\leq \frac{1}{K} \sum_{i = 0}^{K-1} ||\rvg_i||^2 \\
&\leq \frac{2}{Kt} \sum_{i = 0}^{K-1} \frac{\loss(\theta_{i-1}) - \loss(\theta_{i})}{(1 - \cos^2(\phi_{12, i}))}
\end{align*}

If at any iteration, $\cos(\phi_{12, k}) = -1$, then the optimization will stop at that point. If $\forall k \in [0, K]$, $\cos(\phi_{12, k}) \geq \alpha > -1$, then, we have:

\begin{align*}
\min_{0 \leq k \leq K} || \rvg_k ||^2 &\leq \frac{2}{K (1 - \alpha^2) t} \sum_{i = 0}^{K-1} (\loss(\theta_{i-1}) - \loss(\theta_{i})) \\
&= \frac{2}{K (1 - \alpha^2) t} (\loss(\theta_{0}) - \loss(\theta_{K})) \\
&\leq \frac{2}{K (1 - \alpha^2) t} (\loss(\theta_{0}) - \loss^*).
\end{align*}
where $\loss^*$ is the minimal function value.
\end{proof}

Note that the convergence rate of PCGrad in the non-convex setting largely depends on the value of $\alpha$ and generally how small $\cos(\phi_{12, k})$ is on average.

\subsection{Proof of Theorem 2}
\label{app:proof2}

\theoremlocal*

\begin{proof}

Note that $\theta^{\text{MT}} = \theta - t\cdot\rvg$ and $\theta^{\text{PCGrad}} = \theta - t(\rvg - \frac{\rvgone \cdot \rvgtwo}{||\rvgone||^2}\rvgone - \frac{\rvgone \cdot \rvgtwo}{||\rvgtwo||^2}\rvgtwo)$. Based on the condition that $\mathbf{H}(\loss; \theta, \theta^{\text{MT}}) \geq \ell\|\rvg\|_2^2$, we first apply Taylor's Theorem to $\loss(\theta^{\text{MT}})$ and obtain the following result:
\begin{align}
    \loss(\theta^{\text{MT}}) &= \loss(\theta) + \rvg^T(-t\rvg) + \int_0^1 (-t\rvg)^T\frac{\nabla^2\loss(\theta+a\cdot(-t\rvg))}{2}(-t\rvg)da \nonumber\\
    &\geq \loss(\theta) + \rvg^T(-t\rvg) + t^2\cdot \frac{1}{2}\ell\cdot\|\rvg\|_2^2 \nonumber\\
    &= \loss(\theta) - t\|\rvg\|_2^2 + \frac{1}{2}\ell t^2\|\rvg\|_2^2 \nonumber\\
    &= \loss(\theta) + (\frac{1}{2}\ell t^2 - t)\|\rvg\|_2^2 \label{eq:mt_bound}
\end{align}
where the first inequality follows from Definition~\ref{def:curvature} and the assumption $\mathbf{H}(\loss; \theta, \theta^{\text{MT}}) \geq \ell\|\rvg\|_2^2$. From equation~\ref{eq:pcgrad_bound}, we have the simplified upper bound for $\loss(\theta^{\text{PCGrad}})$:
\begin{align}
    \loss(\theta^{\text{PCGrad}}) &\leq \loss(\theta) - (1-\cos^2\phi_{12})[(t-\frac{1}{2}Lt^2)\cdot(\|\rvgone\|_2^2+\|\rvgone\|_2^2) + Lt^2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}]\label{eq:pcgrad_bound_simplified}
\end{align}
Apply Equation~\ref{eq:mt_bound} and Equation~\ref{eq:pcgrad_bound_simplified} and we have the following inequality:
\begin{align}
    &\loss(\theta^{\text{MT}}) - \loss(\theta^{\text{PCGrad}}) \geq \loss(\theta) + (\frac{1}{2}\ell t^2 - t)\|\rvg\|_2^2 - \loss(\theta)\nonumber\\
    & + (1-\cos^2\phi_{12})[(t-\frac{1}{2}Lt^2)(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2) + Lt^2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}] \nonumber\\
    &= (\frac{1}{2}\ell t^2 - t)\|\rvgone + \rvgtwo\|_2^2\!\!+\!\! (1-\cos^2\phi_{12})\!\!\left[(t-\frac{1}{2}Lt^2)\!\cdot\!(\|\rvgone\|_2^2\!+\!\|\rvgtwo\|_2^2)\!+\! Lt^2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right]\nonumber\\
    &= \left(\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - \frac{1-\cos^2\phi_{12}}{2}(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2 - 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12})L\right)t^2\nonumber\\
    &- \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right)t\nonumber\\
    &= \left(\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - \frac{1-\cos^2\phi_{12}}{2}\|\rvgone-\rvgtwo\|_2^2L\right)t^2\nonumber\\
    &- \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right)t\nonumber\\
    &= t\cdot\left[\left(\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - \frac{1-\cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L\right)t\right.\nonumber\\
    &\left.- \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right)\right]\label{eq:difference}
\end{align}
Since $\cos\phi_{12} \leq -\Phi(\rvgone, \rvgtwo) =  -\frac{2\|\rvgone\|_2\|\rvgtwo\|_2}{\|\rvgone\|_2^2 + \|\rvgtwo\|_2^2}$ and $\ell \geq \xi(\rvgone, \rvgtwo) = \frac{(1 - \cos^2\phi_{12})(\|\rvgone-\rvgtwo\|_2^2)}{\|\rvgone + \rvgtwo\|_2^2}L$, we have $$\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - \frac{1-\cos^2\phi_{12}}{2}\|\rvgone-\rvgtwo\|_2^2L \geq 0$$ and $$(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12} \geq 0.$$ By the condition that $t \geq \frac{2}{\ell - \xi(\rvgone, \rvgtwo)L} = \frac{2}{\ell - \frac{(1 - \cos^2\phi_{12})\|\rvgone-\rvgtwo\|_2^2}{\|\rvgone + \rvgtwo\|_2^2}L}$ and monotonicity of linear functions, we have the following:
\begin{align}
    &\loss(\theta^{\text{MT}})\!-\!\loss(\theta^{\text{PCGrad}}) \geq [\left(\frac{1}{2}\|\rvgone\!+\!\rvgtwo\|_2^2\ell-\frac{1\!-\!\cos^2\phi_{12}}{2}\!\cdot\!\|\rvgone\!-\!\rvgtwo\|_2^2L\right)\cdot\frac{2}{\ell\!-\! \frac{(1-\cos^2\phi_{12})\|\rvgone-\rvgtwo\|_2^2}{\|\rvgone + \rvgtwo\|_2^2}L}\nonumber\\
    &- \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right)]\cdot t\nonumber\\
    &=[\|\rvgone+\rvgtwo\|_2^2\cdot\left(\ell-\frac{(1-\cos^2\phi_{12})\cdot\|\rvgone-\rvgtwo\|_2^2}{\|\rvgone+\rvgtwo\|_2^2})L\right)\cdot\frac{1}{\ell - \frac{(1 - \cos^2\phi_{12})\|\rvgone-\rvgtwo\|_2^2}{\|\rvgone + \rvgtwo\|_2^2}L}\nonumber\\
    &- \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right)]\cdot t\nonumber\\
    &= \left[\|\rvgone+\rvgtwo\|_2^2 - \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12}+ 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right)\right]\cdot t\nonumber\\
    &=\left[\|\rvgone\|_2^2\!+\!\|\rvgtwo\|_2^2\!+\!2\|\rvgone\|_2\|\rvgtwo\|_2\!\cos\phi_{12}\!-\! \left((\|\rvgone\|_2^2\!+\!\|\rvgtwo\|_2^2)\cos^2\!\phi_{12}\! +\! 2\|\rvgone\|_2\|\rvgtwo\|_2\!\cos\phi_{12}\right)\right]\cdot t\nonumber\\
    &= (1-\cos^2\phi_{12})(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cdot t\nonumber\\
    &\geq 0\nonumber
\end{align}
\end{proof}

\subsection{PCGrad: Sufficient and Necessary Conditions for Loss Improvement}
\label{app:theorem3}

Beyond the sufficient conditions shown in Theorem~\ref{thm:local}, we also present the sufficient and necessary conditions under which PCGrad achieves lower loss after one gradient update in Theorem~\ref{thm:necessary} in the two-task setting.

\begin{restatable}{theorem}{theoremnecessary}
\label{thm:necessary}
Suppose $\loss$ is differentiable and the gradient of $\loss$ is Lipschitz continuous with constant $L > 0$. 
Let $\theta^{\text{MT}}$ and $\theta^{\text{PCGrad}}$ be the parameters after applying one update to $\theta$ with $\rvg$ and PCGrad-modified gradient $\rvg^{\text{PC}}$ respectively, with step size $t > 0$. 
Moreover, assume $\mathbf{H}(\loss; \theta, \theta^{\text{MT}}) \geq \ell\|\rvg\|_2^2$ for some constant $\ell \leq L$, i.e. the multi-task curvature is lower-bounded. Then $\loss(\theta^{\text{PCGrad}}) \leq \loss(\theta^{\text{MT}})$ if and only if 
\begin{itemize}
    \setlength\itemsep{1em}
    \item $-\Phi(\rvgone, \rvgtwo) \leq \cos\phi_{12} < 0$
    \item $\ell \leq \xi(\rvgone, \rvgtwo)L$
    \item $0 < t \leq \frac{(\|\rvgone\|^2_2 + \|\rvgtwo\|^2_2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}}{\frac{1}{2}\|\rvgone + \rvgtwo\|_2^2\ell - \frac{1 - \cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L}$
\end{itemize} or
\begin{itemize}
    \setlength\itemsep{1em}
    \item $\cos\phi_{12} \leq -\Phi(\rvgone, \rvgtwo)$
    \item $\ell \geq \xi(\rvgone, \rvgtwo)L$
    \item $t \geq \frac{(\|\rvgone\|^2_2 + \|\rvgtwo\|^2_2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}}{\frac{1}{2}\|\rvgone + \rvgtwo\|_2^2\ell - \frac{1 - \cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L}.$
\end{itemize}
\end{restatable}

\vspace{-0.3cm}
\begin{proof}
To show the necessary conditions, from Equation~\ref{eq:difference}, all we need is
\begin{align}
    &t\cdot[(\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - \frac{1-\cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L)t\nonumber\\
    &- \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right)] \geq 0
\end{align}
Since $t \geq 0$, it reduces to show
\begin{align}
    &(\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - \frac{1-\cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L)t\nonumber\\
    &- \left((\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}\right) \geq 0\label{eq:necessary_cond}
\end{align}
For Equation~\ref{eq:necessary_cond} to hold while ensuring that $t \geq 0$, there are two cases:
\begin{itemize}
    \item $\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - (1-\cos^2\phi_{12})(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)L \geq 0$,\\
    $(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12} \geq 0$,\\
    $t \geq \frac{(\|\rvgone\|^2_2 + \|\rvgtwo\|^2_2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}}{\frac{1}{2}\|\rvgone + \rvgtwo\|_2^2\ell - \frac{1 - \cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L}$
    \item $\frac{1}{2}\|\rvgone+\rvgtwo\|_2^2\ell - (1-\cos^2\phi_{12})(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)L \leq 0$,\\
    $(\|\rvgone\|_2^2+\|\rvgtwo\|_2^2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12} \leq 0$,\\
    $t \geq \frac{(\|\rvgone\|^2_2 + \|\rvgtwo\|^2_2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}}{\frac{1}{2}\|\rvgone + \rvgtwo\|_2^2\ell - \frac{1 - \cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L}$
\end{itemize}
, which can be simplified to
\begin{itemize}
    \item $\cos\phi_{12} \leq -\frac{2\|\rvgone\|_2\|\rvgtwo\|_2}{\|\rvgone\|_2^2 + \|\rvgtwo\|_2^2} = -\Phi(\rvgone, \rvgtwo)$,\\
    $\ell \geq \frac{(1 - \cos^2\phi_{12})(\|\rvgone\|_2^2 + \|\rvgtwo\|_2^2)}{\|\rvgone + \rvgtwo\|_2^2}L = \xi(\rvgone, \rvgtwo)$,\\
    $t \geq \frac{(\|\rvgone\|^2_2 + \|\rvgtwo\|^2_2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}}{\frac{1}{2}\|\rvgone + \rvgtwo\|_2^2\ell - \frac{1 - \cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L}$
    \item $-\frac{2\|\rvgone\|_2\|\rvgtwo\|_2}{\|\rvgone\|_2^2 + \|\rvgtwo\|_2^2} = -\Phi(\rvgone, \rvgtwo) \leq \cos\phi_{12} < 0$,\\
    $\ell \leq \frac{(1 - \cos^2\phi_{12})(\|\rvgone\|_2^2 + \|\rvgtwo\|_2^2)}{\|\rvgone + \rvgtwo\|_2^2}L = \xi(\rvgone, \rvgtwo)$,\\
    $0 < t \leq \frac{(\|\rvgone\|^2_2 + \|\rvgtwo\|^2_2)\cos^2\phi_{12} + 2\|\rvgone\|_2\|\rvgtwo\|_2\cos\phi_{12}}{\frac{1}{2}\|\rvgone + \rvgtwo\|_2^2\ell - \frac{1 - \cos^2\phi_{12}}{2}(\|\rvgone-\rvgtwo\|_2^2)L}$.
\end{itemize}

The sufficient conditions hold as we can plug the conditions to RHS of Equation~\ref{eq:necessary_cond} and achieve non-negative result.
\end{proof}
\vspace{-0.3cm}

\subsection{Convergence of PCGrad with Momentum-Based Gradient Descent}
\label{app:momentum}

In this subsection, we show convergence of PCGrad with momentum-based methods, which is more aligned with our practical implementation. In our analysis, we consider the heavy ball method~\cite{polyak1964some} as follows: $$\theta_{k+1} \leftarrow \theta_k - \alpha_k \nabla\loss(\theta_k) + \beta_k (\theta_k - \theta_{k-1})$$ where $k$ denotes the $k$-th step and $\alpha_k$ and $\beta_k$ are step sizes for the gradient and momentum at step $k$ respectively. We now present our theorem.

\begin{restatable}{theorem}{momentum}
\label{thm:momentum}
Assume $\loss_1$ and $\loss_2$ are $\mu_1$- and $\mu_2$-strongly convex and also $L_1$- and $L_2$-smooth respectively where $\mu_1, \mu_2, L_1, L_2 > 0$. Define $\phi^k_{12}$ as the angle between two task gradients $\rvgone{(\theta_k)}$ and $\rvgtwo{(\theta_k)}$ and define $R_k = \frac{\|\rvgone(\theta_k)\|}{\|\rvgtwo(\theta_k)\|}$. Denote $\mu_k = (1 - \cos\phi^k_{12}/R_k)\mu_1 + (1 - \cos\phi^k_{12}\cdot R_k)\mu_2$ and $L_k = (1 - \cos\phi^k_{12}/R_k)L_1 + (1 - \cos\phi^k_{12}\cdot R_k)L_2$
Then, the PCGrad update rule of the heavy ball method with step sizes $\alpha_k = \frac{4}{\sqrt{L_k} + \sqrt{\mu_k}}$ and $\beta_k = \max\{|1 - \sqrt{\alpha_k\mu_k}|,|1 - \sqrt{\alpha_kL_k}|\}^2$ will converge linearly to either (1) a location in the optimization landscape where $\cos(\phi^k_{12}) = -1$ or (2) the optimal value $\loss(\theta^*)$.
\end{restatable}

\begin{proof}
We first observe that the PCGrad-modified gradient $\rvg^{\text{PC}}$ has the following identity:
\begin{align}
    \rvg^\text{PC} &= \rvg - \frac{\rvgone \cdot \rvgtwo}{||\rvgone||^2}\rvgone - \frac{\rvgone \cdot \rvgtwo}{||\rvgtwo||^2}\rvgtwo\nonumber\\
    &= (1 - \frac{\rvgone \cdot \rvgtwo}{||\rvgone||^2})\rvgone + (1 - \frac{\rvgone \cdot \rvgtwo}{||\rvgtwo||^2})\rvgtwo\nonumber\\
    &= (1 - \frac{\rvgone \cdot \rvgtwo}{\|\rvgone\|\|\rvgtwo\|}\frac{\|\rvgtwo\|}{\|\rvgone\|})\rvgone + (1 - \frac{\rvgone \cdot \rvgtwo}{\|\rvgone\|\|\rvgtwo\|}\frac{\|\rvgone\|}{\|\rvgtwo\|})\rvgtwo\nonumber\\
    &= (1 - \cos\phi_{12} / R)\rvgone + (1 - \cos\phi_{12}\cdot R)\rvgtwo\label{eq:split}.
\end{align}
Applying Equation~\ref{eq:split}, we can write the PCGrad update rule of the heavy ball method in matrix form as follows:
\begin{align*}
    \left\|\begin{bmatrix}
    \theta_{k+1} - \theta^*\\
    \theta_k - \theta^*
    \end{bmatrix}\right\|_2 &= \left\|\begin{bmatrix}
    \theta_{k} + \beta_k(\theta_k - \theta_{k-1}) -  \theta^* \\
    \theta_k - \theta^*
    \end{bmatrix} -  \alpha_k\begin{bmatrix}
    \rvg^{\text{PC}}(\theta_k) \\
    0
    \end{bmatrix}\right\|_2\\
    &= \left\|\begin{bmatrix}
    \theta_{k} + \beta_k(\theta_k - \theta_{k-1}) -  \theta^* \\
    \theta_k - \theta^*
    \end{bmatrix}\right.\\
    &\left.-  \alpha_k\begin{bmatrix}
    (1 - \cos\phi^k_{12}/R_k)\rvgone(\theta_k) + (1 - \cos\phi^k_{12}\cdot R_k)\rvgtwo(\theta_k) \\
    0
    \end{bmatrix}\right\|_2\\
    &= \left\|\begin{bmatrix}
    \theta_{k} + \beta_k(\theta_k - \theta_{k-1}) -  \theta^* \\
    \theta_k - \theta^*
    \end{bmatrix}\right.\\
    &\left.- \alpha_k\begin{bmatrix}
    \left[(1 - \cos\phi^k_{12}/R_k)\nabla^2\mathcal{L}_1(z_k) + (1 - \cos\phi^k_{12}\cdot R_k)\nabla^2\mathcal{L}_2(z'_k)\right](\theta_k -  \theta^*) \\
    0
    \end{bmatrix}\right\|_2\\
    &\text{for some }z_k,  z'_k\text{ on the line segment between }\theta_k\text{ and }\theta^*\\
    &=\left\|\begin{bmatrix}
    (1+\beta_k)I-\alpha_kH_k & -\beta_k I\\
    I & 0
    \end{bmatrix}\begin{bmatrix}
    \theta_k -  \theta^*\\
    \theta_{k-1} - \theta^*
    \end{bmatrix}\right\|_2\\
    &\leq \left\|\begin{bmatrix}
    (1+\beta_k)I-\alpha_kH_k & -\beta_k I\\
    I & 0
    \end{bmatrix}\right\|_2\left\|\begin{bmatrix}
    \theta_k-\theta^*\\
    \theta_{k-1}-\theta^*
    \end{bmatrix}\right\|_2
\end{align*}
where $H_k = (1 - \cos\phi^k_{12}/R_k)\nabla^2\mathcal{L}_1(z_k) + (1 - \cos\phi^k_{12} \cdot R_k)\nabla^2\mathcal{L}_2(z'_k)$.

By strong convexity and smoothness of $\loss_1$ and $\loss_2$, we have the eigenvalues of $\nabla^2\mathcal{L}_1(z_k)$ are between $\mu_1$ and $L_1$. Similarly, the eigenvalues of $\nabla^2\mathcal{L}_2(z'_k)$ are between $\mu_2$ and $L_2$. Thus the eigenvalues of $H_k$ are between $\mu_k = (1 - \cos\phi^k_{12}/R_k)\mu_1 + (1 - \cos\phi^k_{12}\cdot R_k)\mu_2$ and $L_k = (1 - \cos\phi^k_{12}/R_k)L_1 + (1 - \cos\phi^k_{12}\cdot R_k)L_2$~\cite{fulton2000eigenvalues}. Hence following Lemma 3.1 in ~\cite{notes}, we have $$\left\|\begin{bmatrix}
    (1+\beta_k)I-\alpha_kH_k & -\beta_k I\\
    I & 0
    \end{bmatrix}\right\|_2 \leq \max\{|1 - \sqrt{\alpha_k\mu_k}|,|1 - \sqrt{\alpha_kL_k}|\}.$$
Thus we have
\begin{align}
    \left\|\begin{bmatrix}
    \theta_{k+1} - \theta^*\\
    \theta_k - \theta^*
    \end{bmatrix}\right\|_2 &\leq \max\{|1 - \sqrt{\alpha_k\mu_k}|,|1 - \sqrt{\alpha_kL_k}|\}\left\|\begin{bmatrix}
    \theta_k-\theta^*\\
    \theta_{k-1}-\theta^*
    \end{bmatrix}\right\|_2\nonumber\\
    &= \frac{\sqrt{\kappa_k}-1}{\sqrt{\kappa_k}+1}\left\|\begin{bmatrix}
    \theta_k-\theta^*\\
    \theta_{k-1}-\theta^*
    \end{bmatrix}\right\|_2\label{eq:sub}\\
    &\leq \left\|\begin{bmatrix}
    \theta_k-\theta^*\\
    \theta_{k-1}-\theta^*
    \end{bmatrix}\right\|_2\nonumber
\end{align}
where $\kappa_k = \frac{L_k}{\mu_k}$ and Equation~\ref{eq:sub} follows from substitution $\alpha_k = \frac{4}{\sqrt{L_k} + \sqrt{\mu_k}}$. Hence PCGrad with heavy ball method converges linearly if $\cos\phi^k_{12} \neq -1$.
\end{proof}


==> Gradient Surgery for Multi-Task Learning NeurIPS/related_work.tex <==
\section{Related Work}

Algorithms for multi-task learning typically consider how to train a single model that can solve a variety of different tasks~\citep{caruana97multitask, bakker2003clustering, ruder2017overview}.
The multi-task formulation has been applied to many different settings, including supervised learning~\citep{zhang2014facial, long2015learning, yang2016trace, sener2018multi, zamir2018taskonomy} and reinforcement-learning~\citep{espeholt2018impala, wilson2007multi}, as well as many different domains, such as vision~\citep{bilen2016integrated, misra2016cross, kokkinos2017ubernet, liu2018attention, zamir2018taskonomy}, language~\citep{collobert2008unified, dong2015multi, mccann2018natural, radford2019language} and robotics~\citep{riedmiller2018learning, wulfmeier2019regularized, hausman2018learning}.
While multi-task learning has the promise of accelerating acquisition of large task repertoires, in practice it presents a challenging optimization problem, which has been tackled in several ways in prior work.

A number of architectural solutions have been proposed to the multi-task learning problem based on multiple modules or paths~\citep{fernando2017pathnet, devin2016modularnet, misra2016crossstitch, rusu2016progressive, rosenbaum2017routing, vandenhende2019branched, rosenbaum2017routing}, or using attention-based architectures~\citep{liu2018attention, maninis2019attention}. Our work is agnostic to the model architecture and can be combined with prior architectural approaches in a complementary fashion.
A different set of multi-task learning approaches aim to decompose the problem into multiple local problems, often corresponding to each task, that are significantly easier to learn, akin to divide and conquer algorithms~\citep{levine2016end,rusu2015policydistillation,parisotto2015actor,teh2017distral, ghosh2017dnc, czarneki2019distilling}. 
Eventually, the local models are combined into a single, multi-task policy using different distillation techniques (outlined in~\citep{hinton2015distilling,czarneki2019distilling}).
In contrast to these methods, we propose a simple and cogent scheme for multi-task learning that allows us to learn the tasks simultaneously using a single, shared model without the need for network distillation.


Similarly to our work, a number of prior approaches have observed the difficulty of optimization in multi-task learning~\citep{hessel2019popart, kendall2018multitask, schaul2019ray, suteu2019regularizing}. Our work suggests that the challenge in multi-task learning may be attributed to what we describe as the tragic triad of multi-task learning (i.e., conflicting gradients, high curvature, and large gradient differences), 
which we address directly by introducing a simple and practical algorithm that deconflicts gradients from different tasks. Prior works combat optimization challenges by rescaling task gradients ~\cite{sener2018multi,chen2018gradnorm}. We alter both the magnitude and direction of the gradient, which we find to be critical for good performance (see Fig.~\ref{fig:rl_results}). 
Prior work has also used the cosine similarity between gradients to define when an auxiliary task might be useful~\citep{du2018aux} or when two tasks are related~\cite{suteu2019regularizing}. We similarly use cosine similarity between gradients to determine if the gradients between a pair of tasks are in conflict. %
Unlike~\citet{du2018aux}, we use this measure for effective multi-task learning, instead of ignoring auxiliary objectives.
Overall, we empirically compare our approach to a number of these prior approaches~\cite{sener2018multi,chen2018gradnorm,suteu2019regularizing}, and observe superior performance with PCGrad.
%

\arxiv{Multiple approaches to continual learning have studied how to prevent gradient updates from adversely affecting previously-learned tasks through various forms of gradient projection\icmllast{~\citep{lopez2017gradient, agem, farajtabar2019orthogonal, guo2020improved}}. These methods focus on sequential learning settings, and solve for the gradient projections using quadratic programming~\citep{lopez2017gradient}, only project onto the normal plane of the average gradient of past tasks~\citep{agem}, or project the current task gradients onto the orthonormal set of previous task gradients~\citep{farajtabar2019orthogonal}. In contrast, our work focuses on positive transfer when simultaneously learning multiple tasks, does not require solving a QP, and \emph{iteratively} projects the gradients of each task instead of \emph{averaging} \icmllast{or only projecting the \emph{current} task gradient.}} Finally, our method is distinct from and solves a different problem than the projected gradient method~\citep{gradient_projection}, which is an approach for constrained optimization that projects gradients onto the constraint manifold. 

